DUAL-GLOW: Conditional Flow-Based Generative Model for Modality Transfer

Positron emission tomography (PET) imaging is an imaging modality for diagnosing a number of neurological diseases. In contrast to Magnetic Resonance Imaging (MRI), PET is costly and involves injecting a radioactive substance into the patient. Motivated by developments in modality transfer in vision, we study the generation of certain types of PET images from MRI data. We derive new flow-based generative models which we show perform well in this small sample size regime (much smaller than dataset sizes available in standard vision tasks). Our formulation, DUAL-GLOW, is based on two invertible networks and a relation network that maps the latent spaces to each other. We discuss how given the prior distribution, learning the conditional distribution of PET given the MRI image reduces to obtaining the conditional distribution between the two latent codes w.r.t. the two image types. We also extend our framework to leverage 'side' information (or attributes) when available. By controlling the PET generation through 'conditioning' on age, our model is also able to capture brain FDG-PET (hypometabolism) changes, as a function of age. We present experiments on the Alzheimers Disease Neuroimaging Initiative (ADNI) dataset with 826 subjects, and obtain good performance in PET image synthesis, qualitatively and quantitatively better than recent works.

==> Introduction.tex <==
\section{Introduction}

PET imaging plays an promising role in the early diagnosis of Alzheimer's Disease (AD). AD study is one of the most popular topic in Neuroscience. Compared with other imaging techniques, PET imaging can detect the amyloid-$\beta$ deposition several years before the onset of clinical symptoms \cite{marcus2014brain}, which is important for the early intervention treatment of AD. 

Though PET imaging show great benefits in AD diagnosis, it can be very expensive and time consuming. It requires the expensive cyclotron machine to produce radioactive rays. Besides, it would take one and half hours to finish imaging analogizing half hours for MRI. 

Medical image generation is a challenging task. Compared to natural images, medical images exhibit huge individual variability and large ambiguity, which poses great challenges to faithfully generate reliable images. 

In Glow, the authors showed that the flow-based models can generate sharp facial images with desired properties, such as smiling altitude and eye openness. It shows superior above other generative models through ... . Expressed by it's great performance, we extend the flow-based models in Glow to generate medical images. In Glow, there is only one dataset of images. In our setting, we are interested in generating images with a condition given by the previous images. For example, with a given MRI image, we are interested in how to generate PET image according to it. There exists some previous works in medical image generation, which has used ... . Though they ..., we are the first to use the flow-based generation models for medical images and we are the first to generate images with conditions from other images. 

Medical image generation has extensively studied in recent years \cite{li2014deep, kang2015prediction, wolterink2017deep,nie2017medical,maspero2018dose,han2017mr,pan2018synthesizing}. Existing methods based on deep learning can be divided into two categories: Deep CNNs and Generative Adversarial Networks (GANs). For CNNs, they usually use the U-Net structure to leverage the local information and obtain the good performance. However, since their object is to minimize the loss in Euclidean space (L-$1$, L-$2$), the generator would produce blurry outputs \cite{nie2017medical}. Recently, GANs obtain great scussess in natural image synthesis \cite{brock2018large}, which can generate sharp images via a minimax two-player game \cite{goodfellow2014generative}. Despite its success, GANs usually suffer from the "mode collapse" that tends to produce limited varieties of samples\cite{che2016mode,arjovsky2017wasserstein}. It would get worse since the medical images show the similar anatomical structure. 

Flow-based methods that maximize the likelihood \cite{dinh2014nice,dinh2016density,kingma2018glow} shows great potential in medical image generation.

1. invertible
2. hierarchical : joint the code in this level
3. symmetric
4. 3D

Contribution: 
\begin{itemize}
    \item We achieve the PET generation from MRI, which indicates the great potential in study and clinical use of Alzheimer's Disease.
    \item We propose a novel image generation model called Dual Glows, which can do the conditional image generation.
      
\end{itemize}


\begin{figure}[t]
   %\vspace{-7mm}
\begin{center}
   \centerline{\includegraphics[width=1.05\linewidth]{framework.png}}
\end{center}
\vspace{-8mm}
   \caption{The framework of Conditional Dual Glows.}
\label{fig:framework}
\end{figure}

==> expfig.tex <==
%%% suvr
%\begin{figure}[]
%	\centering
%	\includegraphics[width=0.98\columnwidth]{./figs/suvr.eps}
%	\caption{\label{fig:suvr} The relative SUVRs for 16 ROIs. }
%\end{figure}


%%% mae
%\begin{figure}[]
%	\includegraphics[width=0.98\columnwidth]{./figs/corr.pdf}
%	\caption{\label{fig:exp2} Mean absolute error on held out test set generations, stratified by age, sex, and disease status.}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% demogra %%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[]
%	\centering
%	\begin{subfigure}{7.5cm}
%		\centering\includegraphics[width=7.5cm]{./figs/demogra-1.png}
%	\end{subfigure}
%	\begin{subfigure}{5.5cm}
%		\centering\includegraphics[width=5.5cm]{./figs/demogra-2.png}
%	\end{subfigure}
%	\caption{\label{fig:demographics} Demographics of all individuals included in our experiments. All information was collected from metadata provided by ADNI.}
%\end{figure}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% samples %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% ADs
\begin{figure*}[]
	\centering
	\begin{tabular}{ccc|ccc}
		MRI & GroundTruth & Synthetic & MRI & GroundTruth & Synthetic \\
		
		%%%%%%%%%%%%%%  s
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/1_1_s.png}
		\end{subfigure}&
	\begin{subfigure}{2.cm}
		\centering\includegraphics[width=2.cm]{./figs/1_2_s.png}
	\end{subfigure}&
\begin{subfigure}{2.cm}
	\centering\includegraphics[width=2.cm]{./figs/1_3_s.png}
\end{subfigure}&

	\begin{subfigure}{2.cm}
	\centering\includegraphics[width=2.cm]{./figs/4_1_s.png}
\end{subfigure}&
\begin{subfigure}{2.cm}
	\centering\includegraphics[width=2.cm]{./figs/4_2_s.png}
\end{subfigure}&
\begin{subfigure}{2.cm}
	\centering\includegraphics[width=2.cm]{./figs/4_3_s.png}
\end{subfigure} \\

	
		%%%%%%%%%%%%%%  a
			\begin{subfigure}{2.cm}
		\centering\includegraphics[width=2.cm]{./figs/1_1_a.png}
	\end{subfigure}&
	\begin{subfigure}{2.cm}
		\centering\includegraphics[width=2.cm]{./figs/1_2_a.png}
	\end{subfigure}&
	\begin{subfigure}{2.cm}
		\centering\includegraphics[width=2.cm]{./figs/1_3_a.png}
	\end{subfigure}&
	
	\begin{subfigure}{2.cm}
		\centering\includegraphics[width=2.cm]{./figs/4_1_a.png}
	\end{subfigure}&
	\begin{subfigure}{2.cm}
		\centering\includegraphics[width=2.cm]{./figs/4_2_a.png}
	\end{subfigure}&
	\begin{subfigure}{2.cm}
		\centering\includegraphics[width=2.cm]{./figs/4_3_a.png}
	\end{subfigure} \\
	
	
	%%%%%%%%%%%%%%  c
			\begin{subfigure}{2.cm}
	\centering\includegraphics[width=2.cm]{./figs/1_1_c.png}
\end{subfigure}&
\begin{subfigure}{2.cm}
	\centering\includegraphics[width=2.cm]{./figs/1_2_c.png}
\end{subfigure}&
\begin{subfigure}{2.cm}
	\centering\includegraphics[width=2.cm]{./figs/1_3_c.png}
\end{subfigure}&

\begin{subfigure}{2.cm}
	\centering\includegraphics[width=2.cm]{./figs/4_1_c.png}
\end{subfigure}&
\begin{subfigure}{2.cm}
	\centering\includegraphics[width=2.cm]{./figs/4_2_c.png}
\end{subfigure}&
\begin{subfigure}{2.cm}
	\centering\includegraphics[width=2.cm]{./figs/4_3_c.png}
\end{subfigure} \\

	\end{tabular}


	\caption{\label{fig:samples-ad} Synthetic images are meaningful for subjects in both
		extremes of disease spectrum. Two synthetic AD subjects. From left to right: input of MRI, the ground truth, the synthetic subject.}
\end{figure*}





%%%% CNs
\begin{figure*}[]
	\centering
	\begin{tabular}{ccc|ccc}
		MRI & GT & Synthetic & MRI & GT & Synthetic \\
		
		%%%%%%%%%%%%%%  s
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/2_1_s.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/2_2_s.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/2_3_s.png}
		\end{subfigure}&
		
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/5_1_s.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/5_2_s.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/5_3_s.png}
		\end{subfigure} \\
		
		
		%%%%%%%%%%%%%%  a
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/2_1_a.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/2_2_a.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/2_3_a.png}
		\end{subfigure}&
		
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/5_1_a.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/5_2_a.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/5_3_a.png}
		\end{subfigure} \\
		
		
		%%%%%%%%%%%%%%  c
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/2_1_c.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/2_2_c.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/2_3_c.png}
		\end{subfigure}&
		
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/5_1_c.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/5_2_c.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/5_3_c.png}
		\end{subfigure} \\
		
	\end{tabular}
	
	
	\caption{\label{fig:samples-cn} Two synthetic CN subjects. From left to right: input of MRI, the ground truth, the synthetic subject.}
\end{figure*}



%%%% MCIs
\begin{figure*}[]
	\centering
	\begin{tabular}{ccc|ccc}
		MRI & GT & Synthetic & MRI & GT & Synthetic \\
		
		%%%%%%%%%%%%%%  s
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/3_1_s.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/3_2_s.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/3_3_s.png}
		\end{subfigure}&
		
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/6_1_s.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/6_2_s.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/6_3_s.png}
		\end{subfigure} \\
		
		
		%%%%%%%%%%%%%%  a
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/3_1_a.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/3_2_a.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/3_3_a.png}
		\end{subfigure}&
		
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/6_1_a.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/6_2_a.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/6_3_a.png}
		\end{subfigure} \\
		
		
		%%%%%%%%%%%%%%  c
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/3_1_c.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/3_2_c.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/3_3_c.png}
		\end{subfigure}&
		
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/6_1_c.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/6_2_c.png}
		\end{subfigure}&
		\begin{subfigure}{2.cm}
			\centering\includegraphics[width=2.cm]{./figs/6_3_c.png}
		\end{subfigure} \\
		
	\end{tabular}
	
	
	\caption{\label{fig:samples-mci} Two synthetic MCI subjects. From left to right: input of MRI, the ground truth, the synthetic subject.}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% t-test %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[]
	\centering
	\begin{subfigure}{3.1cm}
		\includegraphics[height=3.cm]{./figs/ttest-a.png}
	\end{subfigure}
	\begin{subfigure}{4.15 cm}
		\includegraphics[height=3.cm]{./figs/ttest-s.png}
	\end{subfigure}
	\begin{subfigure}{4.1 cm}
		\includegraphics[height=3.cm]{./figs/ttest-c.png}
	\end{subfigure}
	\caption{\label{fig:t-test} T-test for generated images(Purple red) and the ground truth (Yellow) in testing data. The large overlapping region illustrates the consistence in AD $\mid$ CN hypothesis testing.}
\end{figure*}



%\begin{figure}[]
%	\centering
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  input
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/1_1_s.png}
%	\end{subfigure}
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/2_1_s.png}
%	\end{subfigure}
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/3_1_s.png}
%	\end{subfigure}
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/4_1_s.png}
%	\end{subfigure}
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/5_1_s.png}
%	\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/6_1_s.png}
%\end{subfigure}
%	
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% GT s
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/1_2_s.png}
%	\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/2_2_s.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/3_2_s.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/4_2_s.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/5_2_s.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/6_2_s.png}
%\end{subfigure}
%	
%	
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% rc s
%	\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/1_3_s.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/2_3_s.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/3_3_s.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/4_3_s.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/5_3_s.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/6_3_s.png}
%\end{subfigure}
%	
%	
%	
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% GT a
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/1_2_a.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/2_2_a.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/3_2_a.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/4_2_a.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/5_2_a.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/6_2_a.png}
%\end{subfigure}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% rc a
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/1_3_a.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/2_3_a.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/3_3_a.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/4_3_a.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/5_3_a.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/6_3_a.png}
%\end{subfigure}
%
%
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% GT c
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/1_2_c.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/2_2_c.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/3_2_c.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/4_2_c.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/5_2_c.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/6_2_c.png}
%\end{subfigure}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% rc c
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/1_3_c.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/2_3_c.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/3_3_c.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/4_3_c.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/5_3_c.png}
%\end{subfigure}
%\begin{subfigure}{2.cm}
%	\centering\includegraphics[width=2.cm]{./figs/6_3_c.png}
%\end{subfigure}
%
%
%	\caption{\label{fig:samples} The first row is the input of MRI. The second row is the GroundTruth for PET images, the third row is the generated images.}
%\end{figure}





%%%%%conditional samples

\begin{figure*}[t]
	\centering
	%\vspace{-8mm}
	\begin{tabular}{C{3mm} ccccccc}
		& MRI & 50 & 60 & 70 & 80 & 90 & 100 \\
		%%%%%%%%%%%%%%%%%%%%% ADs%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%  s&
		&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_7_s_cond.png}
		\end{subfigure} &
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_1_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_2_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_3_s_cond.png}
		\end{subfigure}&
		
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_4_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_5_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_6_s_cond.png}
		\end{subfigure}\\
		
		
		%%%%%%%%%%%%%%  a
		\multirow{3}{*}{AD}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_7_a_cond.png}
		\end{subfigure} &
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_1_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_2_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_3_a_cond.png}
		\end{subfigure}&
		
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_4_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_5_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_6_a_cond.png}
		\end{subfigure}\\
		
		
		%%%%%%%%%%%%%%  c
		&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_7_c_cond.png}
		\end{subfigure} &
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_1_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_2_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_3_c_cond.png}
		\end{subfigure}&
		
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_4_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_5_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/3_6_c_cond.png}
		\end{subfigure}\\
		
		\vspace{-3mm}
		\\
		
		\hline
		\vspace{-3mm}
		\\
		
		%%%%%%%%%%%%%%%%%%%%% MCI %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%  s
		&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_7_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_1_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_2_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_3_s_cond.png}
		\end{subfigure}&
		
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_4_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_5_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_6_s_cond.png}
		\end{subfigure} \\
		
		
		%%%%%%%%%%%%%%  a
		\multirow{3}{*}{MCI}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_7_a_cond.png}
		\end{subfigure} &
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_1_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_2_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_3_a_cond.png}
		\end{subfigure}&
		
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_4_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_5_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_6_a_cond.png}
		\end{subfigure}\\
		
		
		%%%%%%%%%%%%%%  c
		&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_7_c_cond.png}
		\end{subfigure} &
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_1_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_2_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_3_c_cond.png}
		\end{subfigure}&
		
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_4_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_5_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/1_6_c_cond.png}
		\end{subfigure}\\
		
		
		\vspace{-3mm}
		\\
		
		\hline
		\vspace{-3mm}
		\\
		%%%%%%%%%%%%%%%%%%%%% CN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%  s
		&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_7_s_cond.png}
		\end{subfigure} &
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_1_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_2_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_3_s_cond.png}
		\end{subfigure}&
		
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_4_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_5_s_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_6_s_cond.png}
		\end{subfigure}\\
		
		
		%%%%%%%%%%%%%%  a
		\multirow{3}{*}{CN}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_7_a_cond.png}
		\end{subfigure} &
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_1_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_2_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_3_a_cond.png}
		\end{subfigure}&
		
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_4_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_5_a_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_6_a_cond.png}
		\end{subfigure}\\
		
		
		%%%%%%%%%%%%%%  c
		&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_7_c_cond.png}
		\end{subfigure} &
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_1_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_2_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_3_c_cond.png}
		\end{subfigure}&
		
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_4_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_5_c_cond.png}
		\end{subfigure}&
		\begin{subfigure}{1.5cm}
			\centering\includegraphics[width=1.5cm]{./figs/2_6_c_cond.png}
		\end{subfigure}\\
		
	\end{tabular}
	
	
	\caption{\label{fig:cond_samples} Age information manipulation. There are 3 subjects, AD, MCI, and CN, each subject provides $6$ results \textit{w.r.t.} a variant of age labels.}
\end{figure*}


\begin{figure*}[h]
	\centering
	\includegraphics[width=.8\textwidth]{./figs/cond_quan.eps}
	\vspace{-4mm}
	\caption{\label{fig:cond_quan} The mean intensity of $12$ ROIs with the change of age for $3$ average subjects.}
\end{figure*}

%%%%%%conditional samples
%\begin{figure}[]
%	\centering
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/c-0.png}
%	\end{subfigure}
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/c-2.png}
%	\end{subfigure}
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/c-4.png}
%	\end{subfigure}
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/c-6.png}
%	\end{subfigure}
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/c-8.png}
%	\end{subfigure}
%	\begin{subfigure}{2.cm}
%		\centering\includegraphics[width=2.cm]{./figs/c-10.png}
%	\end{subfigure}
%	\caption{\label{fig:cond_samples} The synthesis PET images with different group labels and the same MRI subject. From left to right: CN, SMC, EMCI, MCI, LMCI, AD}
%\end{figure}



%%%%% samples
%\begin{figure}[]
%\centering
%  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/1-gm.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/2-gm.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/3-gm.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/4-gm.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/5-gm.png}
%  \end{subfigure}
%  
%  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/1-gt.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/2-gt.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/3-gt.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/4-gt.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/5-gt.png}
%  \end{subfigure}
%  
%  
%  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/1-r.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/2-r.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/3-r.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/4-r.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/5-r.png}
%  \end{subfigure}
%  
%  
%  
%  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/6-gm.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/7-gm.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/8-gm.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/9-gm.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/10-gm.png}
%  \end{subfigure}
%  
%  
%    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/6-gt.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/7-gt.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/8-gt.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/9-gt.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/10-gt.png}
%  \end{subfigure}
%  
%  
%      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/6-r.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/7-r.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/8-r.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/9-r.png}
%  \end{subfigure}
%  \begin{subfigure}{2.cm}
%    \centering\includegraphics[width=2.cm]{./figs/10-r.png}
%  \end{subfigure}
%  
%\caption{\label{fig:samples} The first row is the input of MRI with gray matter. The second row is the GroundTruth for PET images, the third row is the generated images.}
%\end{figure}
